What is Fair? Defining Fairness in Machine Learning for Health

Ensuring that machine learning (ML) models are safe, effective, and equitable across all patients is critical for clinical decision-making and for preventing the amplification of existing health disparities. In this work, we examine how fairness is conceptualized in ML for health, including why ML models may lead to unfair decisions and how fairness has been measured in diverse real-world applications. We review commonly used fairness notions within group, individual, and causal-based frameworks. We also discuss the outlook for future research and highlight opportunities and challenges in operationalizing fairness in health-focused applications.

==> archived/old_101624.tex <==
%Ensuring that machine learning (ML) models are safe, effective, and equitable across all patient groups is critical for clinical decision-making and for preventing the reinforcement of existing healthcare disparities. This review examines key fairness concepts in ML for healthcare, including the sources of bias in ML models and a comparison of commonly used fairness metrics. It is enriched with real-world examples and features a case study using an openly available electronic health record (EHR) dataset. Additionally, we highlight current challenges and outline future research directions.


%We explain why models can be unfair, provide a summary and comparison of fairness used in the literature, and discuss challenges and future research directions. We also illustrate group fairness principles through a case study of mortality prediction in a publicly available electronic health record dataset.and effective within all patient groups, and do not disadvantage particular patients, is essential to clinical decision making and to prevent the reinforcement of existing healthcare inequities. 

%\noindent \textbf{Objective:} Ensuring that machine learning (ML) algorithms are safe and effective within all patient groups, and do not disadvantage particular patients, is essential to clinical decision making and preventing the reinforcement of existing healthcare inequities. The objective of this tutorial is to introduce the medical informatics community to the common notions of fairness within ML, focusing on clinical applications and implementation in practice. \\

%\noindent \textbf{Target Audience:} As gaps in fairness arise in a variety of healthcare applications, this tutorial is designed to provide an understanding of fairness, without assuming prior knowledge, to researchers and clinicians who make use of modern clinical data. \\

%\noindent \textbf{Scope:} We describe the fundamental concepts and methods used to define fairness in ML, including an overview of why models in healthcare may be unfair, a summary and comparison of the metrics used to quantify fairness, and a discussion of some ongoing research.  We illustrate some of the fairness methods introduced through a case study of mortality prediction in a publicly available electronic health record dataset. Finally, we provide a user-friendly \texttt{R} package for comprehensive group fairness evaluation, enabling researchers and clinicians to assess fairness in their own ML work. 

==> old_051325.tex <==
\blue{In certain cases,  when one fairness criterion is a relaxation of another, multiple fairness metrics can potentially be evaluated together. For example, equalized odds requires both equal false positive and false negative rates across protected groups, whereas equal opportunity requires only equal false negative rates. Evaluating both can provide valuable complementary insights. Using lung cancer screening as an example\cite{seyyed-kalantari_chexclusion_2020}, while equal opportunity ensures that no group is systematically underdiagnosed, equalized odds additionally ensures that no group is systematically overdiagnosed either, which can lead to unnecessary follow-ups and stress. However, it is difficult for a model to satisfy multiple fairness metrics across different categories.}

%In Supplementary Section 4, we also explore the practical implications of these incompatibilities through a case study using an openly available EHR dataset.
%\cite{denis_fairness_2023,bell2023possibility}. 

https://fairware.cs.umass.edu/papers/Verma.pdf

. 

satisfied when the model yields identical decisions for individuals who differ only in their protected attributeIt is a causality-based fairness metric that examines whether changing a protected attribute causes a change in the model's output, holding all else equal.

%However, removing protected attributes from a model warrants careful consideration in health-focused applications. 

Here we introduce a key notion of individual fairness called {\it{fairness through awareness}} (FTA).  FTA was one of the first works on individual fairness and formalized the notion of similarity by defining metrics that measure the distance between individuals and their predictions.

\footnote{\blue{We use the term model's decision here lightly in our toy example. In practice, a model's decision is almost always coupled with human judgement.}}

Notable examples include work on clinical risk prediction and treatment allocation, where causal frameworks have been used to assess fairness with respect to gender, race, and age \cite{pfohl_counterfactual_2019, zhang_causal_2024}.

In our 30-day hospital readmission example, a principal stratum could be a ``dangerous group", that is,  a group of patients who will be readmitted regardless of the model’s decision. Another stratum could be a ``safe group" comprised of patients who will not be readmitted regardless of the model's decision. The remaining strata would include patients whose readmission aligns with the model’s decisions and contradicts with the model’s decisions. Principal fairness is achieved if, within each stratum, the probability of receiving a particular treatment is independent of protected attributes. 

\subsubsection{\blue{Counterfactual Fairness}}
We introduce one way of incorporating causality into fairness through counterfactuals, which are simply ``what-if'' statements. In the context of evaluating fairness, the counterfactual is often the unobserved model's decision that would have happened if the protected attribute had been different \cite{kusner_counterfactual_2017, fawkes2022selection, bynum2024new}.  One of the first counterfactual-based fairness criteria, simply called (individual) {\it{counterfactual fairness}}, deems a model fair if the observed and counterfactual predictions align for an individual when their protected attribute is changed, given all other features are held constant\footnote{Counterfactual fairness may also viewed as an individual fairness criteria as it is grounded in achieving similar treatment for similar individuals\cite{kusner_counterfactual_2017}.} \cite{kusner_counterfactual_2017}.\\

To better explain this concept, consider an over-simplified view of the world in predicting 30-day hospital readmission. The directed acyclic graph (DAG) in Figure \ref{fig:dag} illustrates that the model's decision for 30-day hospital readmission is directly related to previous diagnoses, age, and prescriptions, while race indirectly influences the decision through its impact on access to healthcare, which in turn influences historical diagnoses \cite{pfohl_counterfactual_2019}. When predicting 30-day hospital readmission, counterfactual fairness is satisfied if a Black patient receives the same prediction they would have received if they were counterfactually of a different race, given all other variables are held constant. The \textit{ceteris paribus} condition here is crucial, as in reality healthcare utilization may differ within different communities defined by race, which could influence the rate of 30-day hospital readmission in practice. \blue{A challenge to causal fairness criteria is that they require a working causal model, the assumptions of which cannot be verified from observational data \cite{kusner_counterfactual_2017, salimi2019interventional, fawkes2022selection}. Moreover, issues of identifiability can also arise (i.e., situations where causality-based fairness notions cannot be measured uniquely from the data) and we refer readers to the work of Makhlouf et al.\ for further discussion of this topic \cite{makhlouf2022survey}.} \\

Numerous other estimands from the causal inference literature have been proposed \blue{to quantify fairness and common notions are summarized in Table \ref{tab:causal}. }For example, \textit{counterfactual parity} which measures a population-level, rather than a individual-level, causal effect of the protected attribute on the model's decision \cite{pearl2009causality, mitchell_algorithmic_2021, alves_survey_2023}. \blue{In our example, this means that the overall proportion of predicted readmission would stay the same if everyone's race were counterfactually altered. In other words, the model's decision should not causally depend on race at the population level.} \textit{Conditional counterfactual fairness} is a weaker criteria that considers the total effect of the protected attribute on the decision conditional on a set of variables of interest \cite{kusner_counterfactual_2017}. In our previous example, this means that for each group of individuals with identical characteristics, the 30-day hospital readmission does not change if their race were counterfactually altered. \\

\blue{Additionally, several extensions of group fairness criteria have been developed using counterfactual reasoning. For example, Pfohl et al. proposed an individual level extension of equalized odds based on counterfactuals to evaluate clinical prediction algorithms across gender, race and age groups \cite{pfohl_counterfactual_2019}. Their criterion, \textit{individual equalized counterfactual odds}, is satisfied if the same prediction is made for a patient and counterfactual patient, provided the observed and counterfactual outcomes do not differ. In our example, this means that for all patients whose outcomes remain the same (e.g., both are readmitted) before and after their race is counterfactually changed (e.g., from Black to White), the model should assign the same prediction. These and related criteria, such as \textit{counterfactual equalized odds} and \textit{counterfactual predictive parity}, are mathematically defined in Table \ref{tab:causal}.   }

\subsubsection{\blue{Principal Fairness}}
\blue{Another criterion that has been used in health-focused applications is \textit{principal fairness}, which uses the concept of principal stratification from the causal inference literature.  Principal fairness is population-level fairness criterion that evaluates decisions among individuals who would be similarly impacted by a model's decisions  \cite{imai_principal_2023}. More formally, a model satisfies principal fairness if the model’s decision is conditionally independent of the protected attributes of interest within each principal stratum.  The principal strata are subgroups of patients who share the same potential outcomes under all possible decisions.  When considering binary outcomes with binary decisions, there are typically four principal strata.  \textit{Conditional principal fairness} relaxes this criterion by conditioning on a set of variables of interest such as clinical profiles.  In the hospital readmission example, principal fairness means that ``similar'' individuals, where similarity id defined by the potential outcomes, are predicted to be readmitted at the same rate across groups defined by race. Conditional principal fairness defines similarity in terms of the potential outcomes and additional covariates, such as age or prescriptions.}\\ 

 \blue{While not a ML-focused example, Zhang et al.\cite{zhang_causal_2024} applied principal fairness to assess the fairness of allocation of two treatments for coronary artery disease using EHR data. They defined four principal strata based on patients' potential outcomes of benefiting from (i) treatment 1 only, (ii) treatment 2 only, (iii) both treatments or (iv) neither treatments.  Their analysis revealed notable disparities in treatment allocation across gender and race, suggesting potential unfairness in the clinical decision making.}


 We next provide a brief overview of causal fairness, an increasingly prominent topic in ML that warrants a dedicated review within the health context \cite{loftus2018causal, fawkes2022selection, makhlouf2022survey, carey2022causal, nilforoshan_causal_2022, anderson2024algorithmic, zhang_causal_2024}. As the name suggests, causal fairness focuses on understanding the causal relationships between protected attributes and a model’s decisions \cite{plecko_causal_2024}.  \blue{We review two popular frameworks in causal fairness: \textit{counterfactual fairness} and \textit{principal fairness}. Additional notions of causal fairness such as path-specific fairness, direct and indirect discrimination, principal fairness, and interventional fairness, are detailed in prior work \cite{chiappa_path-specific_2019,nabi_fair_2018,wu_pc-fairness_2019,zhang_causal_2017, zhang_mitigating_2018, ogburn_comment_2019,  wang_blessings_2019, salimi2019interventional, zuo_interventional_2024, zhang_causal_2024}. Although causality-based approaches are especially valuable in health applications for mitigating confounding effects and disentangling mechanisms of bias, the use of causal fairness in health is in its early stages.  As such, we use a toy example to introduce most of the concepts and reference existing real-world examples whenever possible. }\\


 \blue{Counterfactual fairness is built on the idea of a counterfactual, which is simply a ``what-if'' statements.} In the context of evaluating fairness, the counterfactual is often the unobserved model's decision that would have happened if the protected attribute had been different \cite{kusner_counterfactual_2017, fawkes2022selection, bynum2024new}.  

 Figure \ref{fig:dag}

directed acyclic graphs (DAG) fro

To better explain this concept, consider an over-simplified view of the world in predicting 30-day hospital readmission. The directed acyclic graph (DAG) in Figure \ref{fig:dag} illustrates that the model's decision for 30-day hospital readmission is directly related to previous diagnoses, age, and prescriptions, while race indirectly influences the decision through its impact on access to healthcare, which in turn influences historical diagnoses \cite{pfohl_counterfactual_2019}. When predicting 30-day hospital readmission, counterfactual fairness is satisfied if a Black patient receives the same prediction they would have received if they were counterfactually of a different race, given all other variables are held constant. The \textit{ceteris paribus} condition here is crucial, as in reality healthcare utilization may differ within different communities defined by race, which could influence the rate of 30-day hospital readmission in practice. \blue{A challenge to causal fairness criteria is that they require a working causal model, the assumptions of which cannot be verified from observational data \cite{kusner_counterfactual_2017, salimi2019interventional, fawkes2022selection}. Moreover, issues of identifiability can also arise (i.e., situations where causality-based fairness notions cannot be measured uniquely from the data) and we refer readers to the work of Makhlouf et al.\ for further discussion of this topic \cite{makhlouf2022survey}


For Example 2, suppose that $X$ is instead a variable for the residential neighborhood where an individual lives. The key difference between Example 1 and Example 2 is that now $X$ is directly related to $Y$ as neighborhoods with more healthcare infrastructure may have higher readmission capture rates even when underlying frailty is the same.  Higher observed readmission rates in some ZIP codes are not necessarily because patients are more frail, but rather because those locations have better infrastructure. 

Frailty again causes people to be more likely to be re-admitted and to visit the department.  Further, individuals of a particular socioeconomic group are more likely to use the emergency department, not because they are more frail (i.e., $A$ does not impact $U$), but due to structural barriers such as lack of primary care access or insurance coverage. 

These individuals are also no more likely to be readmitted than anyone else with the same level of frailty.  If the model uses $X$ to predict $Y$, it may assign higher predicted probabilities of re-admission to individuals from that group, even though their true risk given $U$ is no higher. In terms of counterfactual fairness, this prediction is considered unfair; changing $A$ while holding $U$ constant would change $X$ and consequently the prediction. In other words, the model’s prediction is sensitive to $A$ in a way that is not justified by underlying differences in health.


{For example, \textit{counterfactual parity} measures a population-level, rather than an individual-level, causal effect of the protected attribute on the model's decision \cite{pearl2009causality, mitchell_algorithmic_2021, alves_survey_2023}. \blue{In our example, this means that the overall proportion of predicted readmission would stay the same if everyone's socioeconomic status were counterfactually altered. In other words, the model's decision should not causally depend on socioeconomic at the population level.} \textit{Conditional counterfactual fairness} is a weaker criteria that considers the total effect of the protected attribute on the decision conditional on a set of variables of interest \cite{kusner_counterfactual_2017}. In our previous example, this means that for each group of individuals with identical characteristics, the 30-day hospital readmission does not change if their race were counterfactually altered.}


Numerous other estimands from the causal inference literature have been proposed \blue{to quantify fairness and common notions are summarized in Table \ref{tab:causal}. }For example, \textit{counterfactual parity} which measures a population-level, rather than a individual-level, causal effect of the protected attribute on the model's decision \cite{pearl2009causality, mitchell_algorithmic_2021, alves_survey_2023}. \blue{In our example, this means that the overall proportion of predicted readmission would stay the same if everyone's race were counterfactually altered. In other words, the model's decision should not causally depend on race at the population level.} \textit{Conditional counterfactual fairness} is a weaker criteria that considers the total effect of the protected attribute on the decision conditional on a set of variables of interest \cite{kusner_counterfactual_2017}. In our previous example, this means that for each group of individuals with identical characteristics, the 30-day hospital readmission does not change if their race were counterfactually altered. \\

\blue{Additionally, several extensions of group fairness criteria have been developed using counterfactual reasoning. For example, Pfohl et al. proposed an individual level extension of equalized odds based on counterfactuals to evaluate clinical prediction algorithms across gender, race and age groups \cite{pfohl_counterfactual_2019}. Their criterion, \textit{individual equalized counterfactual odds}, is satisfied if the same prediction is made for a patient and counterfactual patient, provided the observed and counterfactual outcomes do not differ. In our example, this means that for all patients whose outcomes remain the same (e.g., both are readmitted) before and after their race is counterfactually changed (e.g., from Black to White), the model should assign the same prediction. These and related criteria, such as \textit{counterfactual equalized odds} and \textit{counterfactual predictive parity}, are mathematically defined in Table \ref{tab:causal}.   }


 \begin{figure}[htbp!]
    \centering
    \includegraphics[width = \textwidth]{images/dag.png}
    \caption{\textbf{Directed acyclic graph (DAG) for predicting 30-day hospital readmission}. The DAG illustrates the relationships among various factors influencing the predicted 30-day readmission. Historical diagnoses, age, and prescriptions have a direct influence on predicted 30-day readmission. Race indirectly affects the prediction through access to care, which in turn influences historical diagnoses.}
    \label{fig:dag}
\end{figure}



\begin{table}[h!]
\centering
\renewcommand{\arraystretch}{1.5}
\begin{tabularx}{\textwidth}{|>{\raggedright\arraybackslash}X|>{\raggedright\arraybackslash}X|}
\hline
    \textbf{Metric} & \textbf{Definition}  \\
    \hline
    (Individual) Counterfactual Fairness & $D(a) = D(a')$ for all individuals {\color{blue} and all $a, a' \in \Asc$}\\
    \hline 
    \blue{(Individual) Equalized Counterfactual Odds} & \blue{$P(D(a) = 1 \mid Y(a) = y) = P(D(a') = 1 \mid  Y(a') = y)$ for all individuals, all $y \in \{0,1\}$, and all $a, a' \in \Asc$  } \\
    \hline
    Counterfactual Parity & \blue{$P(D(a) = 1) = P(D(a') = 1)$ for all $a, a' \in \Asc$}\\ 
    \hline
    Conditional Counterfactual Fairness & \blue{$P(D(a) = 1\mid \bZ) = P(D(a') = 1 \mid \bZ)$ for all $a, a' \in \Asc$} \\ 
    \hline
        Counterfactual Equalized Odds & \blue{$P(D = d\mid Y^0 = y, A) = P(D = d\mid Y^0 = y)$ for all $d \in \{0, 1\}$ and $y \in \{0,1\}$} \\
    \hline
    Counterfactual Predictive Parity & \blue{$P(Y^0 = y \mid D =d , A) = P(Y^0 = y \mid D = d)$ for all $d \in \{0, 1\}$ and $y \in \{0,1\}$}  \\
    \hline
    Principal Fairness & \blue{$P(D = d \mid R = r, A) = P(D = d \mid R = r)$ for all $d \in \{0, 1\}$ and $r \in \Rsc$ } \\
    \hline
    Conditional Principal Fairness & \blue{$P(D = d \mid R = r, A, \bZ) = P(D = d \mid R =r , \bZ)$ for all $d \in \{0, 1\}$ and $r \in \Rsc$} \\
    \hline
    \end{tabularx}
    \caption{\textbf{Common Notions of Causal Fairness}. Symbols: $P =$ probability. Notations: $S:$ risk score, $D:$ final prediction based on thresholding $S$, $A:$ protected attribute ($\mathcal{A}$), $D(a)$: prediction with protected attribute $a \in \Asc$, $D(a')$: prediction when protected attribute is counterfactually altered to $a' \in \Asc$, $\bZ$: additional features, $Y^0:$ potential outcome if $D = 0$, $R:$ principal stratum ($\Rsc$).
    }
    \label{tab:causal}
\end{table}


\begin{table}[h!]
\centering
\renewcommand{\arraystretch}{1.4}
\begin{tabular}{|l|l|p{7cm}|}
\hline
\textbf{Metric Name} & \textbf{Mathematical Definition} & \textbf{Textual Meaning} \\
\hline
Counterfactual Fairness & 
$\forall a, a':\ \hat{Y}_{A \leftarrow a}(U) = \hat{Y}_{A \leftarrow a'}(U)$ & 
An individual’s prediction would remain the same had their protected attribute been different, holding all else (latent factors) constant. \\
\hline
Counterfactual Parity & 
$\forall a, a':\ P(\hat{Y} \mid A = a) = P(\hat{Y}_{A \leftarrow a'} \mid A = a)$ & 
For a group with $A = a$, the distribution of predictions is the same as it would be if they had instead had $A = a'$. \\
\hline
Counterfactual Equalized Odds & 
$\forall a, a', y:\ P(\hat{Y}_{A \leftarrow a} \mid Y = y, A = a) = P(\hat{Y}_{A \leftarrow a'} \mid Y = y, A = a)$ & 
Among those with true label $Y = y$ and $A = a$, the prediction distribution is unchanged under counterfactual changes to $A$. \\
\hline
Individualized Equalized Counterfactual Odds & 
$\forall a, a', y:\ \hat{Y}_{A \leftarrow a}(U) = \hat{Y}_{A \leftarrow a'}(U) \mid Y = y$ & 
For an individual with outcome $Y = y$, the prediction is the same in a counterfactual world where $A$ is changed. \\
\hline
Counterfactual Predictive Parity & 
$\forall a, a':\ P(Y \mid \hat{Y}, A = a) = P(Y_{A \leftarrow a'} \mid \hat{Y}, A = a)$ & 
For a given prediction and group $A = a$, the distribution over true labels is the same as it would be if $A$ had been $a'$. \\
\hline
\end{tabular}
\caption{\textbf{Common Notions of Causal Fairness}. Symbols: $P =$ probability. Notations: $S:$ risk score, $D:$ final prediction based on thresholding $S$, $A:$ protected attribute ($\mathcal{A}$), $D(a)$: prediction with protected attribute $a \in \Asc$, $D(a')$: prediction when protected attribute is counterfactually altered to $a' \in \Asc$, $\bZ$: additional features, $Y^0:$ potential outcome if $D = 0$, $R:$ principal stratum ($\Rsc$).
    }
   % \label{tab:causal}
\label{tab:cf_metrics_full}
\end{table}

\begin{table}[h!]
\centering
\renewcommand{\arraystretch}{1.5}
\begin{tabularx}{\textwidth}{|>{\raggedright\arraybackslash}X|>{\raggedright\arraybackslash}X|}
\hline
    \textbf{Metric} & \textbf{Definition}  \\
    \hline
    (Individual) Counterfactual Fairness & $D(a) = D(a')$ for all individuals {\color{blue} and all $a, a' \in \Asc$}\\
    \hline 
    \blue{(Individual) Equalized Counterfactual Odds} & \blue{$P(D(a) = 1 \mid Y(a) = y) = P(D(a') = 1 \mid  Y(a') = y)$ for all individuals, all $y \in \{0,1\}$, and all $a, a' \in \Asc$  } \\
    \hline
    Counterfactual Parity & \blue{$P(D(a) = 1) = P(D(a') = 1)$ for all $a, a' \in \Asc$}\\ 
    \hline
    Conditional Counterfactual Fairness & \blue{$P(D(a) = 1\mid \bZ) = P(D(a') = 1 \mid \bZ)$ for all $a, a' \in \Asc$} \\ 
    \hline
        Counterfactual Equalized Odds & \blue{$P(D = d\mid Y^0 = y, A) = P(D = d\mid Y^0 = y)$ for all $d \in \{0, 1\}$ and $y \in \{0,1\}$} \\
    \hline
    Counterfactual Predictive Parity & \blue{$P(Y^0 = y \mid D =d , A) = P(Y^0 = y \mid D = d)$ for all $d \in \{0, 1\}$ and $y \in \{0,1\}$}  \\
    \hline
    Principal Fairness & \blue{$P(D = d \mid R = r, A) = P(D = d \mid R = r)$ for all $d \in \{0, 1\}$ and $r \in \Rsc$ } \\
    \hline
    Conditional Principal Fairness & \blue{$P(D = d \mid R = r, A, \bZ) = P(D = d \mid R =r , \bZ)$ for all $d \in \{0, 1\}$ and $r \in \Rsc$} \\
    \hline
    \end{tabularx}
    \caption{\textbf{Common Notions of Causal Fairness}. Symbols: $P =$ probability. Notations: $S:$ risk score, $D:$ final prediction based on thresholding $S$, $A:$ protected attribute ($\mathcal{A}$), $D(a)$: prediction with protected attribute $a \in \Asc$, $D(a')$: prediction when protected attribute is counterfactually altered to $a' \in \Asc$, $\bZ$: additional features, $Y^0:$ potential outcome if $D = 0$, $R:$ principal stratum ($\Rsc$).
    }
    \label{tab:causal}
\end{table}

%$P(D_{A \leftarrow a}(U) = d \mid \bX = \bx, A = a) = P(D_{A \leftarrow a'}(U) = d \mid \bX = \bx, A = a)  \quad  \forall a, a' \in \mathcal{A}$ \\

 Simply put, (ii) focuses attention on cases where the protected attribute should not affect the prediction because it does not affect the outcome thereby enabling researchers to discern whether the model is unfairly relying on the protected attribute when it shouldn't. 

  By controlling for frailty and focusing only on cases where the outcome stays the same, we can see whether the model is using socioeconomic status in ways that are not causally relevant to the prediction. 

This helps detect whether the model is using socioeconomic group inappropriately, independent of legitimate pathways (like frailty) that affect the outcome. 

%\begin{table}[ht!]
%    \centering
%    \begin{tabular}{|l|c|} %c|
%    \hline
%        {\bf{Attribute}} & {\bf{Examples}} \\ %& {\bf{Availability in MIMIC-II}} \\
%        \hline
%        Age & \cite{seyyed-kalantari_chexclusion_2020, garriga_machine_2022, schuch_fairness_2023, yfantidou_accuracy_2023} \\ %& \checkmark \\
%        \hline
%        Disability & \cite{garriga_machine_2022} \\ %& \\
%        \hline
%        Marital Status & \cite{wang_comparison_2022} \\ %& \checkmark \\
%        \hline
%        National Origin & \cite{yfantidou_accuracy_2023} \\ %& \\
%        \hline
%        Race & \cite{seyyed-kalantari_chexclusion_2020, wang_comparison_2022,garriga_machine_2022, schuch_fairness_2023, yuan_algorithmic_2023, yfantidou_accuracy_2023, rajkomar_ensuring_2018, wang_bias_2022} \\ %& \checkmark \\
%        \hline
%        Sex & \cite{seyyed-kalantari_chexclusion_2020, wang_comparison_2022,garriga_machine_2022, yuan_algorithmic_2023, yfantidou_accuracy_2023}\\ % & \checkmark \\
%        \hline
%        Socioeconomic Status & \cite{seyyed-kalantari_chexclusion_2020,wang_comparison_2022,schuch_fairness_2023, yfantidou_accuracy_2023, rajkomar_ensuring_2018, wang_bias_2022} \\ %& \checkmark \\
%        \hline
%    \end{tabular}
%    \caption{\textbf{Commonly used protected attributes in machine learning for health.} Examples of studies that evaluate fairness with respect to each protected attribute.}
%\label{tab:protect_attributes}
%\end{table}
( Y = 1 | D = 1 )   = 1 - P(

similar health statuses and hospitalization histories,
it may indicate a lack of Predictive Parity. Such a bias
could lead to unnecessary stress for elderly patients
and their families, increased healthcare  costs, and
inappropriate allocation of resources. To avoid these
biased healthcare decisions, it is important to adjust
the model to ensure that the likelihood of correctly
predicting readmission is equally accurate across age
groups.


Zou et al.\ evaluated conditional use accuracy of models used to predict pulmonary embolisms with data from high-resolution CT scans and EHRs and benchmarked their fairness properties across gender, race/ethnicity, and age.  They 


P

\cite{brandao-de-resende_machine_2023, yang2023algorithmic}. For example, in COVID-19 triage algorithms, conditional use accuracy seeks to ensure that ICU allocations based on the model's decisions are determined by medical needs rather than a protected attribute. Balancing the model's PPV across groups means that patients prioritized for ICU care due to potential severe complications (e.g., high-risk cases) have an equal likelihood of actually experiencing these complications, regardless of protected attributes. Similarly, balancing the NPV across groups ensures that low-risk cases have an equal likelihood of not experiencing complications. 

However, misclassification between proxy and true protected groups introduces bias, in which novel noisy-adjusted fairness metrics may be needed.

While these approaches do not resolve the deeper issues posed by inadequate or biased data, there has been progress toward fairness techniques that operate under such constraints and show promise in health applications \cite{zhang_fairlisa_2023, roy_fairness_2024}. Still, many protected attributes remain excluded from current fairness frameworks, underscoring the need for future methodological innovation that incorporates a wider set of considerations—including privacy, context sensitivity, procedural fairness, and awareness of sociotechnical impacts—alongside inclusive and participatory research practices \cite{tomasev2021fairness}. We see great potential in advancing these directions, especially through efforts aimed at improving data collection and promoting data equity in healthcare settings, as a foundation for fair and responsible decision-making.

Let me know if you'd like this to sound more technical, more accessible, or adapted for a specific type of audience (e.g., grant reviewers, journal editors, etc.).



You’ve hit the Free plan limit for GPT-4o.
Responses will use a \\


For one, most existing fairness definitions were developed outside the health context and may not appropriately capture bias in certain domains\cite{mccoy_ensuring_2020}.  For example, the majority of existing approaches focus on bias due to a single protected attribute and can fall short in complex, real-world applications involving imperfect models, multiple protected attributes, and numerous practical considerations across the ML pipeline (e.g., resource constraints, policy and operational outcomes)\cite{lalor_should_2024}. Secondly,} various protected attributes (e.g., religion, gender identity, and sexual orientation) are often inaccurately measured \blue{or completely missing or only partially observed} due to sociocultural issues and lack of standardized data collection practices \cite{kronk_transgender_2022, ruberg2020data}. \blue{For example, socioeconomic status is not always recorded in observational data, but various proxy variables may be available (e.g., insurance type) \cite{monuteaux2024evaluation}. To address this challenge, \textit{proxy fairness} has been proposed to enable fairness auditing with variables that approximate protected attributes of interest \cite{ guptaProxyFairness2018}.   When protected attributes are unavailable and no suitable proxies exist, fairness metrics that account for missing data may be necessary.}  While by no means a remedy for inadequate data, there has been progress in fairness approaches that operate with limited data on protected attributes and that may prove useful for health applications \cite{zhang_fairlisa_2023, roy_fairness_2024}. To date, however, many protected attributes have been omitted from fairness considerations, which underscores the necessity of future methodological work to acknowledge ``a multiplicity of considerations, from privacy preservation, context sensitivity and process fairness, to an awareness of sociotechnical impact and the increasingly important role of inclusive and participatory research processes'' \cite{tomasev2021fairness}. We anticipate future work in these aforementioned directions,  particularly in strategies focused on data collection and promoting data equity in health contexts, to establish a strong foundation for fair decision-making.\\


 of the MIMIC database containing EHR data from the intensive care unit at Beth Israel Deaconess Medical Status, the Surveillance, Epidemiology, and End Results (SEER) oncology database, and the SUPPORT database of seriously ill hospitalized patients

